A comparison of source term estimators in coupled finite-volume/Monte-Carlo methods with applications to plasma edge simulations in nuclear fusion

In many applications, such as plasma edge simulation of a nuclear fusion reactor, a coupled PDE/kinetic description is required, which is usually solved with a coupled finite-volume/Monte-Carlo method. Different procedures have been proposed to estimate the source terms in the finite volume part that appear from the Monte Carlo part of the simulation. In this paper, we present a systematic comparison of the variance and computational cost of a coherent set of such estimation procedures. We compare the different estimation procedures for mass in a simplified forward-backward scattering model problem, where an analytical comparison is possible, and for mass and momentum in a model problem with realistic scattering. Our results reveal a non-trivial dependence of the optimal choice of estimator on the model parameters and show that different estimation procedures prevail for different quantities of interest.

==> referenties.tex <==
@book{chandrasekhar1950radtransii,
  title={Radiative transfer},
  author={Chandrasekhar, Subrahmanyan},
  year={1950},
  publisher={Oxford University Press}
}

@article{kahn1956MCapplications,
  title={Applications of {M}onte {C}arlo},
  author={Kahn, Herman},
  year={1956},
  publisher={RAND Corporation}
}

%overgenomen uit Maarten zijn phd thesis
@article{braginskii1965transport,
  title={Transport processes in a plasma},
  author={Braginskii, SI},
  journal={Reviews of plasma physics},
  volume={1},
  pages={205},
  year={1965}
}

@article{gelbardondisspanier1966newclassneutrMC,
  title={A new class of {M}onte {C}arlo estimators},
  author={Gelbard, EM and Ondis II, LA and Spanier, J},
  journal={SIAM Journal on Applied Mathematics},
  volume={14},
  number={4},
  pages={697--701},
  year={1966},
  publisher={SIAM}
}

@article{macmillan1966comparisonneutrMC,
  title={Comparison of statistical estimators for neutron {M}onte {C}arlo calculations},
  author={MacMillan, DB},
  journal={Nuclear Science and Engineering},
  volume={26},
  number={3},
  pages={366--372},
  year={1966},
  publisher={American Nuclear Society}
}

@InProceedings{Marshall1966introductorynoteMC,
  title={Introductory note},
  author={Marshall, AW},
  crossref={Meyer1966sympMC},
  pages={1--14}
}

@proceedings{Meyer1966sympMC,
  editor={Meyer, HA},
  title={Symposium on {M}onte {C}arlo Methods},
  booktitle={Symposium on {M}onte {C}arlo Methods (University of Florida, 1954)},
  publisher={Wiley},
  address={New York},
  year={1966}
}

@article{spanier1966twopairsoffamilies,
  title={Two pairs of families of estimators for transport problems},
  author={Spanier, Jerome},
  journal={SIAM Journal on Applied Mathematics},
  volume={14},
  number={4},
  pages={702--713},
  year={1966},
  publisher={SIAM}
}

@article{coveyou1967adjointinMC,
  title={Adjoint and importance in {M}onte {C}arlo application},
  author={Coveyou, Roger R and Cain, VR and Yost, KJ},
  journal={Nuclear Science and Engineering},
  volume={27},
  number={2},
  pages={219--234},
  year={1967},
  publisher={American Nuclear Society}
}

@article{macmillan1967note,
  title={Note on a paper by {J}. {S}panier concerning {M}onte {C}arlo estimators},
  author={MacMillan, DB},
  journal={SIAM Journal on Applied Mathematics},
  volume={15},
  number={2},
  pages={264--268},
  year={1967},
  publisher={SIAM}
}

@article{spanier1970analyticvarred,
  title={An analytic approach to variance reduction},
  author={Spanier, Jerome},
  journal={SIAM Journal on Applied Mathematics},
  volume={18},
  number={1},
  pages={172--190},
  year={1970},
  publisher={SIAM}
}

@article{spanier1971multistage,
  title={A new multistage procedure for systematic variance reduction in {M}onte {C}arlo},
  author={Spanier, Jerome},
  journal={SIAM Journal on Numerical Analysis},
  volume={8},
  number={3},
  pages={548--554},
  year={1971},
  publisher={SIAM}
}

@article{parker1974practicalconsneutrMC,
  title={Practical considerations in solving neutronics problems by the {M}onte {C}arlo method},
  author={Parker, JB},
  journal={Annals of Nuclear Science and Engineering},
  volume={1},
  number={3},
  pages={169--183},
  year={1974},
  publisher={Elsevier}
}

@book{bellman1975ii,
  title={An introduction to invariant imbedding},
  author={Bellman, Richard and Wing, George Milton},
  year={1975},
  publisher={John Wiley \& Sons Inc}
}

@article{amster1976momscoreeqseerste,
  title={Prediction of statistical error in {M}onte {C}arlo transport calculations},
  author={Amster, Harvey J and Djomehri, M Jahed},
  journal={Nuclear Science and Engineering},
  volume={60},
  number={2},
  pages={131--142},
  year={1976},
  publisher={American Nuclear Society}
}

@techreport{kalli1977pointflux,
  title={Evaluation of three {M}onte {C}arlo estimation schemes for flux at a point},
  author={Kalli, HJ and Cashwell, ED},
  year={1977},
  institution={Los Alamos Scientific Lab., N. Mex.(USA)}
}

@article{lux1978standardvarred,
  title={Systematic study of some standard variance reduction techniques},
  author={Lux, I},
  journal={Nuclear Science and Engineering},
  volume={67},
  number={3},
  pages={317--325},
  year={1978},
  publisher={American Nuclear Society}
}

@article{lux1978unifieddef,
  title={Unified definition of a class of {M}onte {C}arlo estimators},
  author={Lux, Iv{\'a}n},
  journal={Nuclear Science and Engineering},
  volume={67},
  number={1},
  pages={107--119},
  year={1978},
  publisher={American Nuclear Society}
}

@article{lux1978remarktracklength,
  title={Remark on the Efficiency of Track-Length Estimators in Reaction Rate Estimations},
  author={Lux, I},
  journal={Nuclear Science and Engineering},
  volume={66},
  number={2},
  pages={258--264},
  year={1978},
  publisher={American Nuclear Society}
}

@article{lux1978remarknonan,
  title={Remark on the theory of nonanalog {M}onte-{C}arlo games},
  author={Lux, I},
  journal={Atomkernenergie},
  volume={31},
  number={3},
  pages={154--155},
  year={1978}
}

@article{booth1979analysis,
  title={Analysis of error in {M}onte {C}arlo transport calculations},
  author={Booth, Thomas E and Cashwell, Edmond D},
  journal={Nuclear Science and Engineering},
  volume={71},
  number={2},
  pages={128--142},
  year={1979},
  publisher={American Nuclear Society}
}

@techreport{lux1979vareff_techrep,
	author={Lux, Iv{\'a}n},
	title={Variance and efficiency in transport, {M}onte {C}arlo Report {KFKI}-1979-35},
	year={1979},
	institution={Central Research Institute for Physics, Budapest, Hungary}
}

@article{sarkar1979scoremomentumIS,
  title={Prediction of statistical error and optimization of biased {M}onte {C}arlo transport calculations},
  author={Sarkar, PK and Prasad, MA},
  journal={Nuclear science and engineering},
  volume={70},
  number={3},
  pages={243--261},
  year={1979},
  publisher={American Nuclear Society}
}

@article{lux1980vareff,
  title={Variance and efficiency in {M}onte {C}arlo transport calculations},
  author={Lux, Iv{\'a}n},
  journal={Computer Physics Communications},
  volume={20},
  number={1},
  pages={119--125},
  year={1980},
  publisher={Elsevier}
}


@article{dawson1983particleincell,
  title={Particle simulation of plasmas},
  author={Dawson, John M},
  journal={Reviews of modern physics},
  volume={55},
  number={2},
  pages={403},
  year={1983},
  publisher={APS}
}

@article{murthy1983optimaltracklbias,
  title={Optimal choice of parameters for tracklength biassing in {M}onte {C}arlo deep-penetration problems},
  author={Murthy, KPN},
  journal={Annals of Nuclear Energy},
  volume={10},
  number={7},
  pages={375--378},
  year={1983},
  publisher={Elsevier}
}

@article{murthy1985asymptotic,
  title={Asymptotic survival probability of random walks on a semi-infinite line},
  author={Murthy, KPN},
  journal={Pramana},
  volume={25},
  number={3},
  pages={231--238},
  year={1985},
  publisher={Springer}
}

@article{murthy1986analyticalvarredleak,
  title={Analytical results of variance reduction characteristics of biased {M}onte {C}arlo for deep-penetration problems},
  author={Murthy, KPN and Indira, R},
  journal={Nuclear Science and Engineering},
  volume={92},
  number={3},
  pages={482--487},
  year={1986},
  publisher={American Nuclear Society}
}
@article{indira1986weightmomentseqexpandscattangl,
  title={Variance reduction under exponential and scattering angle biasing: An analytic approach},
  author={Indira, R and John, TM},
  journal={Nuclear Science and Engineering},
  volume={94},
  number={4},
  pages={323--336},
  year={1986},
  publisher={American Nuclear Society}
}

@article{indira1988weightmomentseqbiased,
  title={Study of biased {M}onte-{C}arlo schemes employing weight-moments equation formulation},
  author={Indira, R},
  journal={Annals of Nuclear Energy},
  volume={15},
  number={2},
  pages={67--74},
  year={1988},
  publisher={Elsevier}
}

@article{indira1988analyticalleakageest,
  title={Analytical study of leakage estimators in {M}onte-{C}arlo simulation of radiation transport},
  author={Indira, R},
  journal={Annals of Nuclear Energy},
  volume={15},
  number={5},
  pages={261--269},
  year={1988},
  publisher={Elsevier}
}

@article{indira1989optimization,
  title={Optimization of biasing parameters in particle transport simulations},
  author={Indira, R},
  journal={Annals of Nuclear Energy},
  volume={16},
  number={11},
  pages={571--576},
  year={1989},
  publisher={Elsevier}
}

@book{lux1991MCPT,
  title={{M}onte {C}arlo particle transport methods: neutron and photon calculations},
  author={Lux, Ivan and Koblinger, L{\'a}szl{\'o}},
  volume={102},
  year={1991},
  publisher={Citeseer}
}

@article{stotler1994degas2,
  title={Neutral gas transport modeling with {DEGAS} 2},
  author={Stotler, Daren and Karney, Charles},
  journal={Contributions to Plasma Physics},
  volume={34},
  number={2-3},
  pages={392--397},
  year={1994},
  publisher={Wiley Online Library}
}

@article{fenstermacher1995uedgedegas,
  title={{UEDGE} and {DEGAS} modeling of the {DIII-D} scrape-off layer plasma},
  author={Fenstermacher, ME and Porter, GD and Rensink, ME and Rognlien, TD and Allen, SL and Hill, DN and Lasnier, CJ and Leonard, T and Petrie, T},
  journal={Journal of nuclear materials},
  volume={220},
  pages={330--335},
  year={1995},
  publisher={Elsevier}
}

@article{raab1999pointflux,
  title={Two new {M}onte {C}arlo methods for point flux estimation},
  author={Raab, A and Beikert, G},
  journal={Computer physics communications},
  volume={123},
  number={1},
  pages={27--45},
  year={1999},
  publisher={Elsevier}
}

@article{mieussens2000discretevel,
  title={Discrete-velocity models and numerical schemes for the {B}oltzmann-{BGK} equation in plane and axisymmetric geometries},
  author={Mieussens, Luc},
  journal={Journal of Computational Physics},
  volume={162},
  number={2},
  pages={429--466},
  year={2000},
  publisher={New York, Academic Press.}
}

@book{stangeby2000plasmaboundary,
  title={The plasma boundary of magnetic fusion devices},
  author={Stangeby, Peter C},
  volume={224},
  year={2000},
  publisher={Institute of Physics Publishing Bristol}
}

@article{barrett2001VRR,
  title={A variationally-based variance reduction method for {M}onte {C}arlo neutron transport calculations},
  author={Barrett, CL and Larsen, EW},
  journal={Annals of Nuclear Energy},
  volume={28},
  number={5},
  pages={457--475},
  year={2001},
  publisher={Elsevier}
}

@article{feng2002emc3,
  title={Transport in island divertors: physics, 3{D} modelling and comparison to first experiments on {W7-AS}},
  author={Feng, Y and Sardei, F and Grigull, P and McCormick, K and Kisslinger, J and Reiter, D and Igitkhanov, Y},
  journal={Plasma physics and controlled fusion},
  volume={44},
  number={5},
  pages={611},
  year={2002},
  publisher={IOP Publishing}
}

@article{densmore2003VRR_mcmc_mcdet,
  title={Variational variance reduction for particle transport eigenvalue calculations using {M}onte {C}arlo adjoint simulation},
  author={Densmore, Jeffery D and Larsen, Edward W},
  journal={Journal of Computational Physics},
  volume={192},
  number={2},
  pages={387--405},
  year={2003},
  publisher={Elsevier}
}

@article{wang2003newenergyfluxmodel,
  title={A new energy flux model in the {DSMC-IP} method for nonequilibrium flows},
  author={Wang, Wen-Lan and Boyd, Iain D},
  journal={AIAA paper},
  volume={3774},
  pages={1-8},
  year={2003}
}

@article{reiter2005eirene,
  title={The {EIRENE} and {B}2-{EIRENE} codes},
  author={Reiter, D and Baelmans, Martine and B{\"o}rner, P},
  journal={Fusion Science and Technology},
  volume={47},
  number={2},
  pages={172--186},
  year={2005},
  publisher={American Nuclear Society}
}

@article{sunboyd2005theoretical,
  title={Theoretical development of the information preservation method for strongly nonequilibrium gas flows},
  author={Sun, Quanhua and Boyd, Iain D},
  journal={AIAA Paper},
  volume={4828},
  pages={1-10},
  year={2005}
}

@article{schwartzentruber2006hybrid,
  title={A hybrid particle-continuum method applied to shock waves},
  author={Schwartzentruber, Thomas E and Boyd, Iain D},
  journal={Journal of Computational Physics},
  volume={215},
  number={2},
  pages={402--416},
  year={2006},
  publisher={Elsevier}
}

@book{spanier1969MCNT,
  title={{M}onte {C}arlo principles and neutron transport problems},
  author={Spanier, Jerome and Gelbard, Ely M},
  year={1969},
  publisher={Addison-Wesley Publishing Company}
}

@article{sun2004hybridrarifiedgas,
  title={A hybrid continuum/particle approach for modeling subsonic, rarefied gas flows},
  author={Sun, Quanhua and Boyd, Iain D and Candler, Graham V},
  journal={Journal of Computational Physics},
  volume={194},
  number={1},
  pages={256--277},
  year={2004},
  publisher={Elsevier}
}

@book{fundamenski2010powerexhaust,
  title={Power exhaust in fusion plasmas},
  author={Fundamenski, Wojciech},
  year={2010},
  publisher={Cambridge University Press}
}

@inproceedings{solomon2011scoremomentumWW,
  title={Verification of the history-score moment equations for weight-window variance reduction},
  author={Solomon, Clell J and Sood, Avneet and Booth, Thomas E and Shultis, J Kenneth},
  booktitle={Proceedings of the International Conference on Mathematics and Computational Methods Applied to Nuclear Science and Engineering (M\&C 2011), Rio de Janeiro, RJ, Brazil},
  year={2011}
}

@techreport{boyddeschenes2011aerospace,
  title={Hybrid particle-continuum numerical methods for aerospace applications},
  author={Boyd, Iain D and Deschenes, Timothy R},
  year={2011},
  institution={DTIC Document}
}

@article{kukushkin2011ITERdivertor,
  title={Finalizing the {ITER} divertor design: the key role of {SOLPS} modeling},
  author={Kukushkin, AS and Pacher, HD and Kotov, V and Pacher, GW and Reiter, D},
  journal={Fusion engineering and design},
  volume={86},
  number={12},
  pages={2865--2873},
  year={2011},
  publisher={Elsevier}
}

@article{booth2012MCmisconceptions,
  title={Common misconceptions in {M}onte {C}arlo particle transport},
  author={Booth, Thomas E},
  journal={Applied Radiation and Isotopes},
  volume={70},
  number={7},
  pages={1042--1051},
  year={2012},
  publisher={Elsevier}
}

@article{rousset2013bacterialchemotaxis,
  title={Simulating individual-based models of bacterial chemotaxis with asymptotic variance reduction},
  author={Rousset, Mathias and Samaey, Giovanni},
  journal={Mathematical Models and Methods in Applied Sciences},
  volume={23},
  number={12},
  pages={2155--2191},
  year={2013},
  publisher={World Scientific}
}

@article{viola2014snowflakevsconv,
  title={Preliminary Comparison of the Conventional and Quasi-Snowflake Divertor Configurations with the 2{D} Code {EDGE}2{D}/{EIRENE} in the {FAST} Tokamak},
  author={Viola, B and Corrigan, G and Harting, D and Maddaluno, G and Mattia, M and Pericoli Ridolfini, V and Zag{\'o}rski, R},
  journal={Contributions to Plasma Physics},
  volume={54},
  number={4-6},
  pages={459--463},
  year={2014},
  publisher={Wiley Online Library}
}%via Kristel haar JCP paper, vb van gebruik van FV/MC

@article{morgan2015weighteddeltatracking,
  title={Weighted-delta-tracking for {M}onte {C}arlo particle transport},
  author={Morgan, LWG and Kotlyar, D},
  journal={Annals of Nuclear Energy},
  volume={85},
  pages={1184--1188},
  year={2015},
  publisher={Elsevier}
}

@book{horton2015iterphys,
  title={{ITER} Physics},
  author={Horton Jr, C Wendell and Benkadda, Sadruddin},
  year={2015},
  publisher={World Scientific}
}

@article{wiesen2015SOLPSITER,
  title={The new {SOLPS}-{ITER} code package},
  author={Wiesen, Sven and Reiter, Detlev and Kotov, Vladislav and Baelmans, Martine and Dekeyser, Wouter and Kukushkin, AS and Lisgo, SW and Pitts, RA and Rozhansky, Vladimir and Saibene, Gabriella and others},
  journal={Journal of Nuclear Materials},
  volume={463},
  pages={480--484},
  year={2015},
  publisher={Elsevier}
}%laatste standaardreferentie naar ITER simulaties

@article{ghoos2016accuracy,
  title={Accuracy and Convergence of Coupled Finite-Volume/{M}onte-{C}arlo Codes for Plasma Edge Simulations},
  author={Ghoos, Kristel and Dekeyser, Wouter and Samaey, Giovanni and B{\"o}rner, Petra and Reiter, Detlev and Baelmans, Martine},
  journal={Contributions to Plasma Physics},
  volume={56},
  number={6-8},
  pages={616--621},
  year={2016},
  publisher={Wiley Online Library}
}

@inproceedings{baeten2017Korea,
	author={Baeten, Matthias and Mortier, Bert and Baelmans, Martine and Samaey, Giovanni},
	title={Improved Correlated Sampling For Iteratively Coupled {PDE}/{M}onte-{C}arlo Methods Used In Plasma Edge Simulations},
	booktitle={Proceedings of the International Conference on Mathematics and Computational Methods Applied to Nuclear Science and Engineering (M\&C 2017), Jeju, Korea},
	year={2017},
}

@article{krasheninnikov2017physicsdetachement,
  title={Physics of ultimate detachment of a tokamak divertor plasma},
  author={Krasheninnikov, SI and Kukushkin, AS},
  journal={Journal of Plasma Physics},
  volume={83},
  number={5},
  year={2017},
  publisher={Cambridge University Press}
}

@article{juno2018discontinuousGalerkinplasma,
  title={Discontinuous {G}alerkin algorithms for fully kinetic plasmas},
  author={Juno, James and Hakim, Ammar and TenBarge, Jason and Shi, E and Dorland, William},
  journal={Journal of Computational Physics},
  volume={353},
  pages={110--147},
  year={2018},
  publisher={Elsevier}
}

@article{mortier2020ii,
	author={Mortier, Bert and Baelmans, Martine and Samaey, Giovanni},
	title={A comparison of source term estimators in coupled finite-volume/{M}onte-{C}arlo methods with applications to plasma edge simulations in nuclear fusion},
	year={2020},
}

@techreport{mortier2020iiappendix,
	author={Mortier, Bert and Baelmans, Martine and Samaey, Giovanni},
	title={Invariant imbedding applied to source term estimation procedures in a simplified {1D0D} slab case},
	year={2020},
	institution={KU Leuven},
	note={https://lirias.kuleuven.be/handle/123456789/658345},
}


@phdthesis{mortier2020phdthesis,
  title={Advanced {M}onte {C}arlo simulation and estimation for kinetic neutral particles in the plasma edge of fusion reactors},
  author={Mortier, Bert},
  year={2020},
  school={KU Leuven, Department of Computer Science}
}

@inproceedings{mortier2017invimb,
  title={An analytical study of Monte Carlo source term estimators in plasma edge simulations of fusion reactors},
  author={Mortier, Bert and Baelmans, Tine and Samaey, Giovanni},
  booktitle={International Conference on Mathematics \& Computational Methods Applied to Nuclear Science \& Engineering, Date: 2017/04/16-2017/04/20},
  year={2017}
}
